Natural Language Proof Checking in Introduction to Proof Classes -- First Experiences with Diproche

We present and analyze the employment of the Diproche system, a natural language proof checker, within a one-semester mathematics beginners lecture with 228 participants. The system is used to check the students' solution attempts to proving exercises in Boolean set theory and elementary number theory and to give them immediate feedback. The benefits of the employment of the system are assessed via a questionnaire at the end of the semester and via analyzing the solution attempts of a subgroup of the students. Based on our results we develop approaches for future improvements.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2021 (ThEdu'21)\\
EPTCS 354, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.354.5}{10.4204/EPTCS.354.5}}
\pdfoutput=1

